Multi-Scale Games: Representing and Solving Games on Networks with Group Structure

Network games provide a natural machinery to compactly represent strategic interactions among agents whose payoffs exhibit sparsity in their dependence on the actions of others. Besides encoding interaction sparsity, however, real networks often exhibit a multi-scale structure, in which agents can be grouped into communities, those communities further grouped, and so on, and where interactions among such groups may also exhibit sparsity. We present a general model of multi-scale network games that encodes such multi-level structure. We then develop several algorithmic approaches that leverage this multi-scale structure, and derive sufficient conditions for convergence of these to a Nash equilibrium. Our numerical experiments demonstrate that the proposed approaches enable orders of magnitude improvements in scalability when computing Nash equilibria in such games. For example, we can solve previously intractable instances involving up to 1 million agents in under 15 minutes.

==> Analysis.tex <==
\section{Equilibrium Analysis under Linear Best Response}\label{sec:analysis} 

In this section, we first introduce a notion of {\em consistency} of the Nash equilibria obtained using different methods. We then analyze strengths and weaknesses of each method both theoretically and numerically (in Section V) using simulation results.

\subsection{Consistency of NE}

\begin{definition}
    We define an action profile in an equilibrium (under multi-scale perspective) to be {\em consistent} if it satisfies
    \begin{equation*}
        \tilde{e}^*_i = e^*_i, \forall i = 1,\cdots,M~, 
    \end{equation*}
where $\tilde{e}_i^*$ is defined in Eqn (\ref{group_br}) and $e_i^* = \sum_{k=1}^{N_i} e_{i,k}^*$, and $e_{i,k}^*$ is defined in Eqn (\ref{eqn:flat_eqb}).
\end{definition}
The notion of consistency concerns whether the group-level game results in the same total effort as the agent-level game. 

\textit{Assumption 1:}     The linear systems in the flat method and the hierarchical method each has a unique feasible solution.
%\end{assumption}

%\com{what Assumption 1 implied in terms of uniqueness of NE. cite appendix.} 
Assumption 1 implies two things. First of all, under the flat network perspective, we can use the flat method to find a unique Nash equilibrium. Secondly, under the multi-scale perspective, the hierarchical method can find a unique Nash equilibrium. Please refer to the appendix for more on conditions that guarantee the existence of unique Nash equilibrium.

\subsection{Unique $c_i^*$ for Consistency}

\begin{theorem}
    Under Assumption 1, there exists a unique value for each group level cost that guarantees the consistency of an equilibrium under the multi-scale perspective. %The unique values are the same in Method 2 and Method 3.
\end{theorem}

\textit{Proof:}

Under Assumption 1, we denote the unique Nash equilibrium under flat network perspective as $\pmb{e}^*_{flat} = \begin{bmatrix} e^*_{1,1} \\ \vdots \\ e^*_{M,N_M} \end{bmatrix}  \succ \pmb{0}$, and denote 
\begin{align} \label{eqn:notation}
	&\pmb{e}^*_{group} = \begin{bmatrix} \sum_{k=1}^{N_1} e^*_{1,k} \\ \vdots \\ \sum_{k=1}^{N_M} e^*_{M,k} \end{bmatrix}, 
	\pmb{e}^*_{ms,i} = \begin{bmatrix} e^*_{i,1} \\ \vdots \\ e^*_{i,N_i} \end{bmatrix}, 
	\pmb{e}^*_{ms} =  \begin{bmatrix} \pmb{e}^*_{flat} \\ \pmb{e}^*_{group} \end{bmatrix};\\
	&\pmb{c}_{group} = \begin{bmatrix} c_1 \\ \vdots \\ c_M \end{bmatrix},
	\pmb{c}_{flat} =  \begin{bmatrix} c_{1,1} \\ \vdots \\ c_{M,N_M} \end{bmatrix},
	\pmb{c}_{ms} = \begin{bmatrix} \pmb{c}_{flat} \\ \pmb{c}_{group} \end{bmatrix}.
\end{align}

When we compare Eqn (\ref{eqn:flat_eqb}) and Eqn (\ref{eqn:flat_br1}) after we replace $e_j$ with $\tilde{e}_j$ (this is how we defined the best responses in the level-1 game), we know that when consistency holds, in the equilibrium, if the agents exert the same level of effort as in the flat game equilibrium $\pmb{e}^*_{flat}$, then they are best responding to each other under the multi-scale perspective as well and we have an equilibrium. Then based on assumption 1, we have
\begin{enumerate}
	\item $\pmb{e}^*_{group}$ is the unique solution to the linear system shown in Eqn (\ref{l2_linsys});
	\item $\pmb{e}^*_{ms,i}$ is the unique solution to the linear system shown in Eqn (\ref{l1_linsys});
	\item $\pmb{e}^*_{ms}$ is the unique solution to the linear system shown in Eqn (\ref{ms_linsys}).
\end{enumerate}


In the hierarchical method, suppose we denote the diagonal component of $H_{ms,G}$ from Eqn (\ref{l2_linsys}) as $-2\textbf{diag}(\pmb{c}_{group})$ and the off-diagonal component is $V$, then we can have, $$H_{ms,G} = -2\textbf{diag}(\pmb{c}_{group}) + V,$$ and then
\begin{align} \label{eqn:unique_ci}
	& -2 \textbf{diag}(\pmb{c}_{group}) \pmb{e}^*_{group} + V \pmb{e}^*_{group} + \pmb{b}_{ms,G} = 0 \nonumber \\
	\Rightarrow ~& 2\textbf{diag}(\pmb{e}^*_{group}) \pmb{c}_{group} = V \pmb{e}^*_{group} + \pmb{b}_{ms,G} \nonumber \\ 
	\Rightarrow ~&\pmb{c}^*_{group} = \frac{1}{2}\textbf{diag}(\pmb{e}^*_{group})^{-1}(V \pmb{e}^*_{group} + \pmb{b}_{ms,G}),
\end{align}
where we use $c_i = c_i^*$ when consistency holds. Therefore, to guarantee consistency, each group level cost is unique in the hierarchical method $(s_1,s_2)$.

We denote the diagonal component of $H_{ms}$ from Eqn (\ref{l1_linsys}) as $-2\textbf{diag}(\pmb{c}_{ms})$, and the off diagonal component as $R_{ms} = H_{ms} + 2\textbf{diag}(\pmb{c}_{ms})$. If we let $c_i = c_i^*$, and investigate Eqn (\ref{ms_linsys}), we have 
\begin{align} \label{eqn:unique_ci1}
    & H_{ms} \pmb{e}^*_{ms}  = \left(-2\textbf{diag}\left(\begin{bmatrix} \pmb{c}_{flat} \\ \pmb{c}^*_{group} \end{bmatrix} \right) + R_{ms} \right) \pmb{e}^*_{ms} = -\pmb{b}_{ms} \\
    \Rightarrow ~& \begin{bmatrix} \pmb{c}_{flat} \\ \pmb{c}^*_{group} \end{bmatrix} = \frac{1}{2}\textbf{diag}(\pmb{e}^*_{ms})^{-1}(R_{ms} \pmb{e}^*_{ms} + \pmb{b}_{ms})
\end{align}
which shows $\pmb{e}^*_{ms}$ solves the linear system shown in Eqn (\ref{ms_linsys}) and thus $c_i = c_i^*$ also corresponds to the unique group level cost in  Hierarchical Method (1,1).
\qed 
%\end{proof}


\begin{theorem}
    Under Assumption 1 and given $c_i = c_i^*$ in Theorem 4.2, then the three methods find the same equilibrium. More precisely, in both $e^*_{flat}$ and $e^*_{ms}$, we have the same $e^*_{i,k}$, for $i=1,\cdots,M$, $k=1,\cdots,N_i$. 
\end{theorem}

The flat method corresponds to the flat network perspective and we only consider $N$ agents and the action profile is of length $N$. While in the hierarchical method, we treat groups as $M$ super-agents and the action profile is of length $M+N$. By the same equilibrium, we mean the individual effort in the equilibrium, $e_{i,k}^*$, being the same. 

The proof of Theorem 4.3 can be done by replacing $e_i^*$ with $\sum e_{i,k}^{*}$ and vice versa. For example, suppose $\pmb{e}^*_{flat}$ solves $H_{flat}\pmb{e}_{flat} + \pmb{b}_{flat} = \pmb{0}$ in Eqn (\ref{flat_linsys}). Then we can get $\pmb{e}_{ms}^*$, $\pmb{e}^*_{ms,G}$, $\pmb{e}^*_{ms,i}, \forall i = 1,\cdots,M$ according to Eqn (\ref{eqn:notation}). Then we can see that $H_{flat}\pmb{e}_{ms}^* + \pmb{b}_{ms} = \pmb{0}$, $H_{ms,G} \pmb{e}^*_{ms,G} + \pmb{b}^*_{ms,G} = \pmb{0}$ and $H_{ms,i}\pmb{e}^*_{ms,i} + \pmb{b}^*_{ms,i} = \pmb{0}$.\\

%Since assumption 1 and $c_i = c_i^*$ imply consistency, 
We can equivalently say that when Assumption 1 and consistency hold at the same time, both the flat method and the hierarchical method can find the same equilibrium. In summary, when Assumption 1 is true, the following three properties are equivalent:
\begin{enumerate}
    \item $c_i = c_i^*$ for $i=1,\cdots,M$;
    \item Consistency holds, $e_i^* = \tilde{e}_i^*$ for $i=1,\cdots,M$;
    \item The flat method and the hierarchical method find the same equilibrium.
\end{enumerate}

We can think of $u_i = g_i(e_i, \pmb{e}_i) + c_i^* e_i^2$ as our higher level characterization for $C_i$. Because with this utility function, it is equivalent for any other agent/super-agent to interact directly with $C_i$ compared with interacting with all individuals in $C_i$.

Note that when multiple equilibria exist under the multi-scale perspective, we can examine consistency of each equilibrium based on the definition. The concept of consistency itself is not restricted to the uniqueness of equilibrium, but it remains an open question whether the different methods will find the same equilibria when Assumption 1 does not hold. 
%However, we are still studying if assumption 1 is not true, the three methods can find the same equilibria or at least some equilibria that are the same.

\subsection{Joint optimization of group costs and effort profile}
Here a natural concern is that we usually don't know the desirable $c_i^*$ a priori.  This motivates a generalization of Algorithm 1, Algorithm 2, that jointly optimizes over the group costs and the effort profile. 

\begin{algorithm}[htbp]
	\SetAlgoLined
	
	Initialize the game, $t_G=0, t_{A_i}=0, i=1,\cdots,M$\;
	\While{$||\pmb{e}-\pmb{e}_{prev}|| > \epsilon$(not converged)}{
		$\pmb{e}_{prev} = \pmb{e}$\;
		\For{$t_2$ = 1 : $s_2$}{
			\If{$t_G > 0$ and $||\tilde{e}_i^{(t_G)} - \tilde{e}_i^{(t_G-1)}|| < \epsilon_G$ (level-2 game converged):}{Break;}
			\For{i = 1 : M:}{
				$\tilde{e}_i^{(t_G+1)} = BR_i(\pmb{\tilde{e}}_{-i}^{(t_G)}, V)$}
			$t_G \leftarrow t_G+1$\;
		}
		
		\For{i = 1 : M}{
			\For{$t_1$ = 1 : $s_1$}{
				\If{$t_{A_i} > 0$ and $||e_{i,k}^{(t_{A_i})} - e_{i,k}^{(t_{A_i}-1)}|| < \epsilon_A$ (the $i$th level-1 game converged)}{Break;}
				\For{k = 1: $N_i$}{
					$e_{i,k}^{(t_{A_i}+1)} = BR_{i,k}(\pmb{e}_{i,-k}^{(t_{A_i})}, W, \pmb{\tilde{e}}^{(t_{G})}, V)$}
				$t_{A_i} \leftarrow t_{A_i}+1$;
			}
	}
$\pmb{c}_{group} = \text{update}(e_1^{(t_{A_1})}, \cdots, e_M^{(t_{A_M})}, V );$
}
	\caption{Hierarchical Method ($s_1, s_2$) and Tune $c_i$}
\end{algorithm} 

In Algorithm 2, the update function of $c_i$ is such that 
\begin{align*}
&~ (V-2\textbf{diag}(\pmb{c}_{group}))\hat{\pmb{e}}^{(t_G)}_{group}+\pmb{b}_{ms,G}\\
\Rightarrow &~ \pmb{c}_{group} = \frac{1}{2}\textbf{diag}(\hat{\pmb{e}}^{(t_G)}_{group})^{-1}(V \hat{\pmb{e}}^{(t_G)}_{group} + \pmb{b}_{ms,G}),
\end{align*}
where 
\begin{equation*}
\hat{\pmb{e}}_{group}^{(t_G)} = \begin{bmatrix}
\sum_{k=1}^{N_1} e_{1,k}^{(t_{A_1})} \\ \vdots \\
\sum_{k=1}^{N_M} e_{M,k}^{(t_{A_M})}
\end{bmatrix},  
\pmb{c}_{group} = \begin{bmatrix}
c_1 \\ \vdots \\ c_M
\end{bmatrix}~. 
\end{equation*}
We show the convergence of Algorithm 2 in the appendix.

Besides using best response dynamics to find the Nash equilibrium, we can also construct convex optimization problems that can jointly optimize group cost and the effort profile to find the consistent NE; please refer to the appendix for more on this.



==> abstract.tex <==
\begin{abstract}
Network or graphical games provide a natural machinery to compactly represent strategic interactions among agents whose payoffs exhibit sparsity in their dependence on the actions of others.
Besides encoding interaction sparsity, however, real networks often exhibit a multi-scale structure, in which agents can be grouped into communities, those communities further grouped, and so on, and where interactions among such groups may also exhibit sparsity.
We present a general model of multi-scale network games that encodes such multi-level structure.
We then develop several algorithmic approaches that leverage this multi-scale structure, and exhibit sufficient conditions for convergence of these to a Nash equilibrium.
Our numerical experiments demonstrate that the proposed approach enables orders of magnitude improvements in scalability of computing Nash equilibria in multi-scale games, and a number of previously intractable instances involving up to 1 million agents that we now solve in under 15 minutes.
\end{abstract}

==> abstract_old.tex <==
% Abstract. Note that this must come before \maketitle.
\begin{abstract}
This paper introduces a multi-scale perspective of network games where group or community structures exist which play a role in agents' strategic interactions.  Specifically, we investigate the case where each agent's utility consists of a local component, much like in a standard network game, and a group component, reflecting the notion where individuals take on a certain group-level identity.  This multi-scale game structure gives rise to an iterative method, switching between the group-stage game and the agent-stage game, for computing the Nash equilibrium of the game, and the issue of consistency between the two games. This paper sets out to provide a precise definition of a class of such multi-scale games and explore whether there are analytical as well as computational advantages to studying the game at both and alternating scales.  Much of our current analysis is done for the case of utility functions with linear best responses. The analysis is also accompanied with some interesting numerical results. The new method we proposed to compute Nash equilibrium using the multi-scale structure of the network can not only find the accurate theoretical result, but also have some computational benefits under certain conditions.
\end{abstract}


==> conclusion_old.tex <==
\section{Conclusion}
In this paper, we investigated network games where group structures exist on the network. Specifically, we investigated the case where each agent's utility consists of a local component and a group component. We demonstrated a multi-scale perspective on the network game and established a corresponding model. Based on the model, we came up with the hierarchical method that utilizes the multi-scale structure to compute the Nash equilibrium of the game. Then, we defined the ``consistency" of an equilibrium under the multi-scale perspective, which is a sufficient condition for the hierarchical method to recover the same equilibrium found under the flat network perspective. Last but not least, we theoretically and numerically analyzed the game under linear best response assumptions and compared the different methods. The analysis showed that the hierarchical method can not only find the accurate theoretical result, but also have computational benefits under certain conditions. 

In future, we have the following directions to generalize and improve our current work:
\begin{enumerate}
	\item Multiple equilibria under both perspectives: we want to investigate games where multiple equilibria exist and for some particular equilibria we can obtain under the flat network perspective, how can we recover them under the multi-scale perspective.
	
	\item More general utility functions: we plan to generalize our findings to a broader class of utility functions with different forms of best responses.
	
	\item An agent's utility not only consists of local component and its own group's utility, but also related to other groups' utilities.
	\begin{align*}
	u_{i,k} = & f_{i,k}(e_{i,k},\pmb{e}_{i,-k})+\alpha_{i,k} \cdot g_i(e_i,\pmb{e}_{-i})
	+ \sum_{j\neq i}\theta_{ij,k} \cdot g_j(e_j,\pmb{e}_{-j}), ~~\text{where}~ \alpha_{i,k} >0, \theta_{ij,k} \geq 0.
	\end{align*}
	An example of this type of utility function can be the utility for some military forces in Ukraine. Suppose each military force is an agent, and all forces in Ukraine form group $C_U$ and all forces in Russia form group $C_R$. Some $a_{U,k}$ might actually prefer the Russia group being strong while some other $a_{U,l}$ wish Russia is weak. This can't be easily characterized with the previous utility function but can be done with the generalized one above.
	
	\item Mechanism Design and Policy Design: We have already seen in Section 5 that when consistency does not hold, the equilibrium will be different under the multi-scale perspective compared with the flat network perspective. We want to see if we can utilize this feature and design good mechanisms or policies that can improve the social welfare or even improve every agent's utility. If such good mechanisms or policies exist, they can be useful tools for multi-scale system design.
\end{enumerate}


==> model-removed.tex <==
\subsection{Utility functions} 
%The utility functions are defined for  level-1 agents. 
For a level-1 agent in an $L$-level game, its utility consists of $L$ components, each representing a level. Entities in the same group on the same level share the same higher level components. Suppose for $a^{(1)}_{i}$, we use $k_l$ to denote the index of its level-$l$ supervisor, and 
% \begin{equation*}
%     i^{(l)} \in S^{(l)}_{i^{(l+1)}}, \forall l = 1,\dots, L, i^{(1)}=i, i^{(L+1)}=1,
% \end{equation*}
its utility is given by 
\begin{equation} \label{eqn:utility}
    u_i(x^{(1)}_i, \pmb{x}^{(1)}_{-i}) = \sum_{l=1}^{L} u^{(l)}_{k_l} \bigg( x^{(l)}_{k_l}, \pmb{x}^{(l)}_{S - k_l} \bigg).
\end{equation}
% We assume that agent $a_i, i \in S_k$ has a utility function $f_i$ of the following form:
%\com{the subscript in the last term is getting very hard to read; maybe we need to consider using parenthesis $x()$ instead. }
%\rev{What about using $\pmb{x}^{(l)}_{S-i}$?}
% \begin{equation} \label{eqn:utility}
%     u_i(x_i, \pmb{x}_{S_k \backslash i}, \pmb{y}_{-k}) = u^{(1)}_i(x_i,\pmb{x}_{S_k \backslash i}) + u^{(2)}_k(y_k,\pmb{y}_{-k}).
% \end{equation}
\rev{To see how the network structure plays a role in our model, consider a utility component $u_i^{(l)} \bigg( x_i^{(l)}, \pmb{x}^{(l)}_{S-i} \bigg)$,  $i \in S_k^{(l)}$, which takes the form:
\begin{equation} \label{eqn:util_component}
    u_i^{(l)} \bigg( x_i^{(l)}, \pmb{x}^{(l)}_{S-i} \bigg) = b_i^{(l)} \bigg( [W_k^{(l)}]_i \cdot \pmb{x}^{(l)}_{S_k^{(l)}} \bigg) - c_i^{(l)} \bigg( x_i^{(l)} \bigg),\nonumber
\end{equation}
where $[W_k^{(l)}]_i$ is the $i$th row of $W_k^{(l)}$. The first component $b_i^{(l)}$ is the benefit term that depends on the local adjacency matrix and the  actions of local neighbors; the second component $c_i^{(l)}$ is the cost term that depends on its own action.
}

\rev{The above utility captures the fact that an agent can benefit from being part of a sequence of nested groups; while a higher-level entity does not take actions, it has a utility ($u^{(l)}_{k_l}$) that depends on the aggregate actions of its members and its peers at the same level through the weighted adjacency matrix at that level.}
%Here $u^{(l)}_{i^{(l)}}$ represents the level-$l$ component of $a^{(1)}_{i}$'s utility. For every level, an entity is affected by individual efforts within its own group and the group's local network topology. Every entity is also affected by actions taken by members of other groups on the same level, but only through their aggregate actions, and is influenced by the higher level network topology. Equivalently, we can think of the aggregate actions as actions taken by higher level entities that represent other groups.
From an agent's point of view, this modeling choice obscures the exact agent-to-agent topology beyond its own group and captures a type of incomplete information at the group level. 

\begin{figure}[htbp]
% 	\centering
	\begin{minipage}{0.18\textwidth}
		\centering
		\includegraphics[width=3.5cm]{Flat_Net.png} % first figure itself
		\caption{Flat Network Perspective.}\label{fig:ex_flat}
	\end{minipage}\hspace{0.2in}
	\begin{minipage}{0.22\textwidth}
		\centering
		\includegraphics[width=4.5cm]{Multi_Scale.png} % second figure itself
		\caption{Multi-Scale.}\label{fig:ex_multi}
	\end{minipage}
\end{figure}

\subsection{Flat game perspective} 

%Below we define three games that correspond to different perspectives of the game. 
%{\bf Full-Game (Flat Game):} 

Given a multi-scale game model, we next show that we can always recover an underlying conventional network game (also referred to as the {\em flat} or {\em full} game) by expanding and redistributing higher-level aggregate actions onto level-1. %, as well as the higher level connections to level-1 connections. 
%thereby availing ourselves  existing methods. 
%An example (4-agent, 2-level) is illustrated in Figure \ref{fig:ex_flat} with 2 level-1 groups, the first highlighted in red and the second in blue. 
For simplicity of notation, We show this using a 2-level  example. If we expand the $\pmb{x}^{(2)}$ terms into $\pmb{x}^{(1)}$ terms in $u^{(2)}_{i^{(2)}}$ in Eqn (\ref{eqn:utility}), then the utility of $a^{(1)}_{i}$ can be expressed as a function of the efforts of all other agents in the network as follows: 
\begin{align} \label{eqn:flat}
    &~ u_{i^{(1)}}(x^{(1)}_{i^{(1)}}, \pmb{x}^{(1)}_{-i^{(1)}}) \nonumber\\
    =&~ u^{(1)}_{i^{(1)}} \bigg( x^{(1)}_{i^{(1)}}, \pmb{x}^{(1)}_{S^{(1)}_{i^{(2)}} \backslash i^{(1)}} \bigg) \nonumber \\
    &~ + u^{(2)}_{i^{(2)}} \bigg( \sigma^{(1)}_1 (\pmb{x}^{(1)}_{S^{(1)}_1}), \cdots, \sigma^{(1)}_{N^{(1)}} (\pmb{x}^{(1)}_{S^{(1)}_{N^{(1)}}}) \bigg)\nonumber \\
    \Leftrightarrow &~ u^{flat}_{i^{(1)}} (x^{(1)}_{i^{(1)}}, \pmb{x}^{(1)}_{-i^{(1)}}) \nonumber\\
    = &~ u^{(1)}_{i^{(1)}} \bigg( x^{(1)}_{i^{(1)}}, \pmb{x}^{(1)}_{S^{(1)}_{i^{(2)}} \backslash i^{(1)}} \bigg) + \tilde{u}^{(2)}_{i^{(2)}} \bigg( \pmb{x}^{(1)}_{S^{(1)}_{i^{(2)}}},\pmb{x}^{(1)}_{-S^{(1)}_{i^{(2)}}} \bigg) \nonumber \\
    = &~ u^{(1)}_{i^{(1)}} \bigg( x^{(1)}_{i^{(1)}}, \pmb{x}^{(1)}_{S^{(1)}_{i^{(2)}} \backslash i^{(1)}} \bigg) + \tilde{u}^{(2)}_{i^{(2)}} \bigg( x^{(1)}_{i^{(1)}},\pmb{x}^{(1)}_{-i^{(1)}} \bigg). 
\end{align}
%\com{suggest using $(2)$ in the superscripts within $u^{(2)}$ in the above so as to be consistent with the general expression in (10).}
%\rev{Should I use an example instead?}
This means that the game can ultimately be represented as a conventional network game, by distributing/spreading the group-level edge weights $W^{(2)}_{km}$ \rev{(embedded in the expression of the utility function $u_i(\cdot)$)} to all pairwise connections between members of groups $S^{(2)}_m$ and $S^{(2)}_k$; this results in a set of revised agent-to-agent edge weights and the removal of the group-to-group edges. 

Specifically, the equivalent edge weight from $a^{(1)}_j, j \in S^{(1)}_m$ to $a^{(1)}_i, i \in S^{(1)}_k$ is now $w^{(2)}_{km}$ and the edge weight from $a^{(1)}_i$ to $a^{(1)}_j$ is now $w^{(2)}_{lk}$, for all $k, l = 1,\dots, N^{(2)}, k \neq l; i, j=1,\dots, N^{(1)}, i\neq j$.
This essentially breaks the group level interactions down to the individual level, and results in a ``full game'' or ``flat game'', which can be analyzed using existing methods developed for conventional network games. 
Figure \ref{fig:ex_flat} gives this flat view of the game consisting of 4 agents and 2 level-1 groups, one highlighted in read, the other blue. We see that each agent is now ``connected'' to all other agents in the network. 

==> related.tex <==
\section{Related Work} \label{sec:related} 
Network games have received increasing attention in recent years. \cite{jackson2015games} and \cite{GPoN2016} provided surveys on recent works in this area.  Below we review some that are most relevant to the present paper.  

Best responses have been used as an analytical tool for equilibrium analysis. Conditions for the existence, uniqueness and stability of the Nash equilibria in network games under general best responses have been studied in \cite{parise2019variational, naghizadeh2017uniqueness, scutari2014real}. The following works \cite{naghizadeh2017uniqueness, scutari2014real} identify that when the Jacobian matrix of the Best response matrix is a P-matrix or is positive definite, then a feasible unique Nash equilibrium exists. As a special case, the uniqueness of Nash equilibria under linear best responses have been studied in \cite{naghizadeh2018provision,LinBRD2008,OptPrice}. Both \cite{naghizadeh2018provision} and \cite{LinBRD2008} identify the strict diagonal dominance of the adjacency matrix as a sufficient condition for the existence of a feasible unique Nash equilibrium. Moreover, the paths to the unique equilibrium is studied in \cite{LinBRD2008}, this work proved the bounded linear best responses will converge to the unique Nash equilibrium for any initialization. Our work introduces two perspectives on the network game and refers the conventional perspective as ``flat network perspective" and define our new perspective using the group structure as ``multi-scale perspective". Previous works on best response and equilibrium analysis are used as references under the flat network perspective. In Section 4 and 5, we extended the analysis of equilibrium and best responses under the multi-scale perspective of a network. 

To the best of the authors' knowledge, previous work on network games that involve group or community structure focus on finding such structures instead of utilizing it as an analytical tool. One line of research focuses on detecting the group/community structures. Community detection in networks using game theoretic methods have been studied in \cite{GTFCD2017, DetecStru2004, CDDSN2014}. Another line of research focus on how agents form groups, \cite{GroupForm2005,FormNetGr2001}. These works provide guidance on how to create multi-scale structure for a network. Our work, however, tries to analyze the network games where the group/community structure is already given, and use the structure as an analytical tool for the analysis on equilibrium and best responses.

%\com{Please revise accordingly.} 
